Convolutional Neural Networks can achieve binary bail judgement classification

There is an evident lack of implementation of Machine Learning (ML) in the legal domain in India, and any research that does take place in this domain is usually based on data from the higher courts of law and works with English data. The lower courts and data from the different regional languages of India are often overlooked. In this paper, we deploy a Convolutional Neural Network (CNN) architecture on a corpus of Hindi legal documents. We perform a bail Prediction task with the help of a CNN model and achieve an overall accuracy of 93\% which is an improvement on the benchmark accuracy, set by Kapoor et al. (2022), albeit in data from 20 districts of the Indian state of Uttar Pradesh.

==> other_1.tex <==
The dataset contains both bail data and non-bail data, we choose to work with only the bail data for our purpose. The bail data is divided into 71 separate JSON files, each for one of the districts of U.P. Each JSON file contains the bail judgements for all the cases from the 2 year time-frame for all district courts in that district. This data is well organized in the JSON files. All the data for each of the district courts within a single district are kept separate with the help of key-value pairs in the files. There is also distinctions among the data from a single district court, in that there are two types of case data in these files. Those which have been processed, these are labelled under the "processed" key, and those which are not processed, labelled under the "valid" key. The difference between these two is that the processed data constitutes those case judgements where each case data has been separated into "header", "body", "result", "decision", "bail\textunderscore amount", and "segments" (which is the body divided into "judge-opinion" and "facts-and-arguments"), while the data under "valid" lacks such division \citep{kapoor-etal-2022-hldc}.

We then went on to extract the data from only the "body", "decision", and "bail\textunderscore amount" for each case data in separate CSV files for each district. 


